Resilience for Multigrid Software at the Extreme Scale

Fault tolerant algorithms for the numerical approximation of elliptic partial differential equations on modern supercomputers play a more and more important role in the future design of exa-scale enabled iterative solvers. Here, we combine domain partitioning with highly scalable geometric multigrid schemes to obtain fast and fault-robust solvers in three dimensions. The recovery strategy is based on a hierarchical hybrid concept where the values on lower dimensional primitives such as faces are stored redundantly and thus can be recovered easily in case of a failure. The lost volume unknowns in the faulty region are re-computed approximately with multigrid cycles by solving a local Dirichlet problem on the faulty subdomain. Different strategies are compared and evaluated with respect to performance, computational cost, and speed up. Especially effective are strategies in which the local recovery in the faulty region is executed in parallel with global solves and when the local recovery is additionally accelerated. This results in an asynchronous multigrid iteration that can fully compensate faults. Excellent parallel performance on a current peta-scale system is demonstrated.

==> 4_localrecoverystrat.tex <==
%!TEX root = ./resilience.tex
%
To avoid the error pollution effect observed in Subsec.\ \ref{sec:FaultModel}, we now propose a first recovery strategy. 
To avoid polluting the healthy subdomain $\Omega_I$ with the large residuals in 
the faulty subdomain $\Omega_F$, we separate the two domains,
that is, we set the faulty subdomain in quarantine
until the lost values in $u_F$  can be recovered by  
solving a local auxiliary
discrete Dirichlet problem 
with  boundary data $u_{\Gamma}$ on $\Gamma$.

Before continuing with the global multigrid iteration  
for solving
\eqref{eq:PoissonLin}, we approximate the 
auxiliary local problem by $n_F$  
steps of a given iterative solver, see
Alg. \ref{alg:LocalAlg}.
%
\begin{algorithm}
\caption{Local recovery (LR) algorithm}\label{alg:LocalAlg}
\begin{algorithmic}[1]
    \State Solve \eqref{eq:PoissonLin} by multigrid cycles.
    \If{Fault has occurred}
    \State \textbf{STOP} solving \eqref{eq:PoissonLin}.
    \State Recover the boundary data $\ul u_{\Gamma_{F}}$ 
from line 4 in  \eqref{eq:algSystemGhost}.
    \State Initialize $\ul u_F$ with zero.
    \State Approximate line 5  in  \eqref{eq:algSystemGhost} by 
solving iteratively with $n_F$ steps:
\State  $\qquad A_{FF} \ul u_F = \ul f_F - A_{F\Gamma_F} \ul u_{\Gamma_F}$
    \State \textbf{RETURN} to line 1 with new values $\ul u_F$ in $\Omega_F$. 
    \EndIf
  \end{algorithmic}
\end{algorithm}

Obviously, this algorithm is only a first step towards a fault
tolerant multigrid solver and suffers from the fact that
during the approximation of the local problem on $\Omega_F$,
the processors assigned to the healthy 
domain $\Omega_I$ will wait idle. 
Since in practice $\Omega_F $ is small compared to $\Omega_I$, 
this will naturally result in many idle processors during the recovery.
This performance loss  
will be addressed in Sec.~\ref{sec:globalrecovery}. 
Nevertheless the local strategies 
will already provide valuable 
insight in the selection of the iterative solver for the  
recovery subproblem and in the choice of $n_F$.

\subsection{Influence of the algorithmic parameters on the performance}\label{sec:AlgoPerf}
To illustrate the method, we consider again the situation of Subsec. \ref{sec:FaultModel}.
We study five different iterative solvers: 
local V-cycles, local W-cycles, local F-cycles, each
with three pre- and post-smoothing steps
of the hybrid Gauss-Seidel smoother presented in Sec. \ref{sec:ModelProblem}, 
Gauss-Seidel relaxation only (Smooth),
and Jacobi preconditioned CG (PCG) iterations,
see the left picture in Fig. \ref{fig:ResiConvLocDiff}. 
On the right, we show the influence of $n_F$ on the
convergence of the global multigrid solver when multigrid cycles are used.
%
\begin{figure}[ht]
\centering
  \input{Figure/faultafter5iterDiffTypes}
  \input{Figure/faultafter5iterDiffVcycles}
  \caption{Convergence of the  relative residual for different local recovery strategies (left) and
         different $n_F$ for local V-cycles (right).}
\label{fig:ResiConvLocDiff}
\end{figure}
%
We observe that  there are huge differences.
The different local multigrid cycles, i.e., V-, W-, and  F-cycle,
perform similarly well.
In these cases, setting $n_F =2$ results in a cycle advantage of $\kappa = 1/5$.
However to obtain a smaller $\kappa$ for PCG, we have to set the number of local iterations
to $n_F \geq 100$.
This becomes % situation is 
even worse  when using local Gauss-Seidel smoothing for recovery.
Here, we report two extreme cases. The first one with
$n_F = 15$ results in a similar computational
cost as the V-cycle % situation 
with $n_F = 2$, but no improvement compared to the do-nothing job can
be observed.
The second one achieves  $\kappa = 1/5$ but 
needs $n_F = 2000$, an absurdly
high computational cost.
Thus, clearly Smooth and PCG are no suitable candidates for solving the local  subproblem.
On the right of Fig. \ref{fig:ResiConvLocDiff},
we show the influence of  $n_F$ for the case of a local V-cycle multigrid solver.
The delay in finding the solution significantly depends on how accurately
the  local recovery problem is solved.
Here performing one local V-cycle for recovery reduces the iterations in the subsequent global 
solution process by two iterations.
Two local V-cycles produce an advantage of three global iterations, 
and three local V-cycles completely compensate the effect of the fault.


Table \ref{tab:DiffFaults} shows
the influence of the iteration type, 
of $k_F$ and $n_F$ on $\kappa$.
We consider three cases for $k_F$, i.e., $k_F   \in \{ 5, 7, 11 \}$, the five iterative solvers from above, and $n_F$ 
ranging from one to $6500$.
%
\begin{table}[ht]
%
  \footnotesize\centering
  \caption[Tab.]{Cycle Advantage for an early (after 5 iterations), middle (after 7 iterations), and late (after 11 iterations) 
		fault for different $n_F$ and iterative solvers.}
  \label{tab:DiffFaults}
  \vspace{1em} 
%
 \begin{tabular}{@{}*{1}{p{65pt}}@{}@{}*{1}{p{30pt}}@{}}
  \toprule
  \multicolumn{2}{c}{\textbf{Fault After 5 Iter.}}\\
  \cmidrule{1-2}
  ~Strategies~~~  &  ~~~~$\kappa$~~~ \\
  \cmidrule(r){1-1}\cmidrule(r){2-2} 
   No Rec		&	0.80	\\
  1 $\times$ Vcycle	&	0.60	\\
  2 $\times$ Vcycle	&	0.20	\\
  3 $\times$ Vcycle	&	0.00	\\
  4 $\times$ Vcycle	&	0.00	\\
%  5 $\times$ Vcycle	&	0.00	\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  1 $\times$ Wcycle	&	0.80		\\
  2 $\times$ Wcycle	&	0.20 		\\
  3 $\times$ Wcycle	&	0.00		\\
  4 $\times$ Wcycle	&	0.00		\\
 % 5 $\times$ Wcycle	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  1 $\times$ Fcycle	&	0.80		\\
  2 $\times$ Fcycle	&	0.60		\\
  3 $\times$ Fcycle	&	0.00		\\
  4 $\times$ Fcycle	&	0.00		\\
 % 5 $\times$ Fcycle	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  50~\, $\times$ PCG 	&	0.80		\\
  100 $\times$ PCG 	&	0.60		\\
  150 $\times$ PCG 	&	0.20		\\
  200 $\times$ PCG 	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  500~\, $\times$ Smooth	&	0.80		\\
  1000 $\times$ Smooth	&	0.60		\\
  2000 $\times$ Smooth	&	0.20		\\
  3000 $\times$ Smooth	&	0.00		\\
  \bottomrule
 \end{tabular}
%
 \hspace{5pt}
 \begin{tabular}{@{}*{1}{p{65pt}}@{}@{}*{1}{p{30pt}}@{}}
  \toprule
   \multicolumn{2}{c}{\textbf{Fault After 7 Iter.}}\\
  \cmidrule{1-2}
 ~Strategies~~~  &  ~~~~$\kappa$~~~ \\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
 No Rec		&	0.86		\\
 1 $\times$ Vcycle	&	0.71		\\
 2 $\times$ Vcycle	&	0.43		\\
 3 $\times$ Vcycle	&	0.29		\\
 5 $\times$ Vcycle	&	0.00		\\
 %7 $\times$ Vcycle	&	0.00		\\
 \cmidrule(r){1-1}\cmidrule(r){2-2}
 1 $\times$ Wcycle	&	0.71		\\
 2 $\times$ Wcycle	&	0.43		\\
 3 $\times$ Wcycle	&	0.29		\\
 5 $\times$ Wcycle	&	0.00		\\
% 7 $\times$ Wcycle	&	0.00 		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
 1 $\times$ Fcycle	&	0.71		\\
 2 $\times$ Fcycle	&	0.43		\\
 3 $\times$ Fcycle	&	0.29		\\
 5 $\times$ Fcycle	&	0.00		\\
 %7 $\times$ Fcycle	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
 50~\, $\times$ PCG	&	0.86		\\	
 100 $\times$ PCG 	&	0.71		\\
 150 $\times$ PCG	&       0.43		\\
 250 $\times$ PCG	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
 500~\, $\times$ Smooth	&	0.86		\\
 1000 $\times$ Smooth	&	0.71		\\
 2000 $\times$ Smooth	&	0.43		\\
 4000 $\times$ Smooth	&	0.00		\\
 \bottomrule
  \end{tabular}
  %
  \hspace{5pt}
   \begin{tabular}{@{}*{1}{p{65pt}}@{}@{}*{1}{p{30pt}}@{}}
  \toprule
  \multicolumn{2}{c}{\textbf{Fault After 11 Iter.}}\\
  \cmidrule{1-2}
 ~Strategies~~~  &  ~~~~$\kappa$~~~\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  No Rec		&	0.91		\\
  1 $\times$ Vcycle	&	0.91		\\
  2 $\times$ Vcycle	&	0.73		\\
  5 $\times$ Vcycle	&	0.36		\\
  9 $\times$ Vcycle	&	0.00		\\
 % 11 $\times$ Vcycle	& 	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  1 $\times$ Wcycle	&	0.91		\\
  2 $\times$ Wcycle	&	0.73		\\
  5 $\times$ Wcycle	&	0.36		\\
  9 $\times$ Wcycle	&	0.00		\\
  %11 $\times$ Wcycle	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  1 $\times$ Fcycle	&	0.91		\\
  2 $\times$ Fcycle	&	0.73		\\
  5 $\times$ Fcycle	&	0.36		\\
  9 $\times$ Fcycle	&	0.00		\\
  %11 $\times$ Fcycle	&	0.00		\\
  \cmidrule(r){1-1}\cmidrule(r){2-2}
  50~\, $\times$ PCG 	&	0.91		\\
  100 $\times$ PCG	&	0.82		\\
  150 $\times$ PCG 	&	0.64		\\
  350 $\times$ PCG 	&	0.00		\\
   \cmidrule(r){1-1}\cmidrule(r){2-2}
  500~\, $\times$ Smooth	&	0.91		\\
  1000 $\times$ Smooth	&	0.82		\\
  2000 $\times$ Smooth	&	0.64		\\
  6500 $\times$ Smooth	&	0.00		\\
   \bottomrule
 \end{tabular}
 %
 \vspace{-0.1cm}
\end{table}
%
In all % our 
settings we achieve $\kappa < 1$.
However, only multigrid cycles can efficiently reduce
$\kappa$. For $n_F = k_F$, we then always find $\kappa=0$.
Note that using local multigrid recovery
leads to the situation that the subsequent global iterations exhibit a favorable
pre-asymptotic behavior that is lacking when other iterative schemes are used for recovery.
We emphasize that this is no coincidence,
but lies inherent in how multigrid methods work.
Since the local multigrid cycles reduce the residual also on coarser levels, they
compute a solution to the local recovery problem that is better suited
for the subsequent global iterations than when a single grid iteration is performed,
even when this is run until the residual is equally small.
Due to this 
pre-asymptotic behavior, we already obtain $\kappa=0$ with $n_F = k_F-2$.
Even with $n_F =50 $ and $n_F=500$ in the case of PCG and Smooth, respectively,
the number of required extra multigrid steps is exactly the same as in a do-nothing job, i.e., only barely reduced to $k_F-1$. 
Only with a further increase of $n_F$ % yields smaller 
the values for the cycle advantage $\kappa$ can be further reduced.
In the case of recovery by Gauss-Seidel smoothing iterations
alone and $k_F=11$,  a ridiculous large number of
$n_F=6500$ would be needed to achieve % does  result in 
a perfect recovery with $\kappa=0$, whereas $n_F= 2000$ still requires 
requires $7$ extra global multigrid steps.

In effect this means that attempting to perform a recovery with Gauss-Seidel  and PCG iterations 
cannot lead to practical recovery algorithms,
just as using a direct solver for the local subproblem
would be too slow to be of use.
In these cases, the time spend to compute the local recovery solution
would be much larger than throwing the complete solution away
and executing the global multigrid iteration from scratch.

\subsection{Extension to Stokes}
The local recovery strategy is not limited to positive definite systems but can
also be applied to saddle-point problems.
As a model problem for an indefinite linear equation system, we consider a stabilized
discretization of Stokes equation. 
We use linear equal-order FE spaces and ensure stability by 
a standard PSPG stabilization for the pressure,
see, e.g., \cite{brezzi-douglas_1988}.
To solve the system efficiently, we apply 
a geometric multigrid method in the pressure and velocity with the same standard inter-grid transfer components as before.
The smoother reflects the indefinite structure and is of
Uzawa-type, see, e.g.,
\cite{bank-welfert-yserentant_1990,schoeberl-zulehner_2003, zulehner_2002}.

In the case of a failure,
we re-compute the values of the velocity and pressure
by local solves of
an auxiliary Stokes problem with Dirichlet
boundary condition. 
In contrast to the standard situation, we also fix the pressure at the boundary $\Gamma$.
To guarantee that the system is uniformly well-posed, we formally 
include a compatibility condition obtained from the normal components of the velocity.
Then the structure of Alg.~\ref{alg:LocalAlg} can be used unmodified. However
some of the details change and as already pointed out,
the multigrid algorithm 
for solving the system has to be adapted to the indefinite nature of the problem. 

In Fig. \ref{fig:FTStokes}, a test case is set up in which after 5 iterations a failure 
of a process interrupts the computation.
We apply different number of local V-cycles to
recover the lost values.
Similar to the positive definite case in Subsec.\ref{sec:AlgoPerf},
a local recovery by $n_F = k_F - 2$ result in $\kappa = 0$.
%
\begin{figure}[ht]
\centering
  \input{Figure/faultStokesSystem}
\caption{Convergence of the relative residual of the Stokes system for different $n_F$.}
\label{fig:FTStokes}
\end{figure}



==> faultStokesSystem.tex <==
\centering
	\pgfplotsset{tick label style ={font=\scriptsize}}
	\begin{tikzpicture}[scale=0.8]
		\begin{semilogyaxis}[
		width=0.6\textwidth,
		height=0.5\textwidth,
		xlabel={Iterations},
		ylabel={Residual},
%		legend pos=south,
		xticklabels = {0, 5, 5, 10, 15, 20},
		xtick = {0, 5, 8, 13, 18, 23},
		ymajorgrids = true,
		xmin = 0, xmax = 25,
		ymin=1e-16,ymax=1,
		ytick = {1e0, 1e-4, 1e-8, 1e-12, 1e-16},
		%yticklabels = {\scriptsize $10^0$,\scriptsize $10^{-4}$,\scriptsize $10^{-8}$,\scriptsize $10^{-12}$,
		%\scriptsize $10^{-16}$},
		legend style={/tikz/every odd column/.style={yshift=2pt}, font=\scriptsize, text height = 0.5ex, legend cell align = left},
%		every axis label/.append style = {font=\tiny}
		]
		\def \sh {3}
		% Before Fault
		 \addplot[color=blue,mark=o] coordinates {
		(0.0, 1                    )
		(1.0, 0.0195858)
		(2.0, 0.00148052)
		(3.0, 0.000207228)
                (4.0, 3.23611E-005)
                (5.0,4.67119E-006)
                };

                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%  After Fault
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\fill[text=FAULT, blue,fill opacity=0.25, ] (axis cs:5,1e-16) rectangle (axis cs: 5+\sh,1);  
	\node[rotate=90] at (axis cs:6.5,1e-8) {\bf FAULT \& RECOVERY};             %\& RECOVERY
	%\node[coordinate, pin = {[rotate=90] right: FAULT}]  at (axis cs:6,1e-8) {};
                % No Fault
                 \addplot+[color=blue,mark=o , mark options = {fill=blue}] coordinates {
                (5 +\sh, 4.67119E-006)
                (6 +\sh, 6.59265E-007)
                (7 +\sh, 9.77949E-008)
                (8 +\sh, 1.53732E-008)
                (9+\sh, 2.63801E-009)
                (10+\sh, 5.04005E-010)
                (11+\sh, 1.04772E-010)
                (12+\sh, 2.3862E-011)
                (13+\sh, 5.60648E-012)
                (14+\sh, 1.3743E-012)
                (15+\sh, 3.41106E-013)
                (16+\sh, 8.65056E-014)
                (17+\sh, 2.21268E-014)
                (18+\sh, 5.8501E-015)
                (19+\sh, 1.93212E-015)
                (20+\sh, 1.29388E-015)
                (21+\sh, 1.23759E-015)
                (22+\sh, 1.23759E-015)
                (23+\sh, 1.23759E-015)
                 };     
        \addplot+[color=red, mark=square, mark options={solid}] coordinates { 
	(5 +\sh, 0.156973   )
         (6 +\sh,0.00191215    )
	 (7 +\sh,8.58045E-005    )
	 (8 +\sh,5.51872E-006    )
	 (9 +\sh,0.000000511    )
	 (10+\sh,6.95966E-008    )
	 (11+\sh,1.20518E-008    )
	 (12+\sh,2.32917E-009    )
	 (13+\sh,4.76556E-010    )
	 (14+\sh,1.0081E-010    )
	 (15+\sh,2.19079E-011    )
	 (16+\sh,4.86718E-012    )
	 (17+\sh,1.1052E-012    )
	 (18+\sh,2.56015E-013    )
	 (19+\sh,6.05563E-014    )
	 (20+\sh,1.46358E-014    )
	 (21+\sh,3.78451E-015    )
	 (22+\sh,1.52173E-015   )
	 (23+\sh,1.25286E-015)
	      };     
                     
                       
                       
                       
                 
                 
                 
                 
                 
                 
        % 1x Vcycle       
        \addplot+[color=green,mark=triangle,mark options={solid}] coordinates { 
% 	 (5 +\sh,	       0.012087)
% 	 (6 +\sh,      0.000281127)
% 	 (7 +\sh,      1.69743E-005)
% 	 (8 +\sh,      2.20963E-006)
% 	 (9 +\sh,      3.77051E-007)
% 	 (10+\sh,      6.62948E-008)
% 	 (11+\sh,      1.1051E-008)
% 	 (12+\sh,      0.000000002)
% 	 (13+\sh,      3.89308E-010)
% 	 (14+\sh,      8.07962E-011)
% 	 (15+\sh,      1.72455E-011)
% 	 (16+\sh,      3.78834E-012)
% 	 (17+\sh,      8.40573E-013)
% 	 (18+\sh,      1.88926E-013)
% 	 (19+\sh,      4.26773E-014)
% 	 (20+\sh,      9.78087E-015)
% 	 (21+\sh,      2.53678E-015)
% 	 (22+\sh,     1.32987E-015)
% 	 (23+\sh,	1.23759E-015)
	 
(5 +\sh,0.0120872)
(6 +\sh,0.000275942)
(7 +\sh,1.41887E-005)
(8 +\sh,1.35924E-006)
(9 +\sh,2.04175E-007)
(10+\sh,3.82402E-008)
(11+\sh,7.70264E-009)
(12+\sh,1.61518E-009)
(13+\sh,3.46312E-010)
(14+\sh,7.5474E-011)
(15+\sh,1.6644E-011)
(16+\sh,3.70404E-012)
(17+\sh,8.3073E-013)
(18+\sh,1.87495E-013)
(19+\sh,4.25477E-014)
(20+\sh,9.77805E-015)
(21+\sh,2.54388E-015)
(22+\sh,1.33659E-015)
(23+\sh,1.23906E-015)
};      1.23289E-015
               
                 
        % 2x Vcycle    
        \addplot+[color=orange,mark=diamond,mark options={solid}] coordinates {         
% (5 +\sh,                  0.00163482	)
% (6 +\sh,		  3.92825E-005  )
% (7 +\sh,		  2.20773E-006  )
% (8 +\sh,		  2.50814E-007  )
% (9 +\sh,		  4.1814E-008   )
% (10+\sh,		  7.52962E-009  )
% (11+\sh,		  1.44229E-009  )
% (12+\sh,		  2.90142E-010  )
% (13+\sh,		  6.13079E-011  )
% (14+\sh,		  1.3256E-011   )
% (15+\sh,		  2.92367E-012  )
% (16+\sh,		  6.51155E-013  )
% (17+\sh,		  1.46477E-013  )
% (18+\sh,		  3.3172E-014   )
% (19+\sh,		  7.65434E-015  )
% (20+\sh,		  2.12682E-015  )
% (21+\sh,		  1.29668E-015  )
% (22+\sh,		  1.23492E-015  )
% (23+\sh,		  1.23076E-015  )
% 

(5 +\sh,0.00163466)
(6 +\sh,3.89256E-005)
(7 +\sh,2.03223E-006)
(8 +\sh,2.02687E-007)
(9 +\sh,3.24564E-008)
(10+\sh,6.27895E-009)
(11+\sh,1.29302E-009)
(12+\sh,2.74719E-010)
(13+\sh,5.94681E-011)
(14+\sh,1.30494E-011)
(15+\sh,2.89265E-012)
(16+\sh,6.46283E-013)
(17+\sh,1.45381E-013)
(18+\sh,3.2906E-014)
(19+\sh,7.57456E-015)
(20+\sh,2.10603E-015)
(21+\sh,1.28986E-015)
(22+\sh,1.28986E-015)
(23+\sh,1.28986E-015)



          };      
                 
         %3x Vcycle
     \addplot+[solid,color=magenta, mark=pentagon,mark options={solid}] coordinates {             
% (5 +\sh,    		0.000270718                 	)
% (6 +\sh,		  		6.73929E-006    )
% (7 +\sh,		  		4.63168E-007    )
% (8 +\sh,		  		6.20566E-008    )
% (9 +\sh,		  		1.01751E-008    )
% (10+\sh,		  		1.91623E-009    )
% (11+\sh,		  		3.85494E-010    )
% (12+\sh,		  		8.19065E-011    )
% (13+\sh,		  		1.78289E-011    )
% (14+\sh,		  		3.96268E-012    )
% (15+\sh,		  		8.92216E-013    )
% (16+\sh,		  		2.0358E-013     )
% (17+\sh,		  		4.69964E-014    )
% (18+\sh,		  		1.10486E-014    )
% (19+\sh,		  		2.87828E-015    )
% (20+\sh,		  		1.37902E-015    )
% (21+\sh,		  		1.24091E-015    )
% (22+\sh,		                1.24091E-015    )
% (23+\sh,		                1.24091E-015   )

(5 +\sh,0.000270932)
(6 +\sh,6.51277E-006)
(7 +\sh,3.89863E-007)
(8 +\sh,0.00000005)
(9 +\sh,8.9365E-009)
(10+\sh,1.79212E-009)
(11+\sh,3.74417E-010)
(12+\sh,8.02739E-011)
(13+\sh,1.74982E-011)
(14+\sh,3.86468E-012)
(15+\sh,8.6231E-013)
(16+\sh,1.94005E-013)
(17+\sh,4.40078E-014)
(18+\sh,1.01272E-014)
(19+\sh,2.62221E-015)
(20+\sh,1.34277E-015)
(21+\sh,1.23793E-015)
(22+\sh,1.23161E-015)
(23+\sh,1.23416E-015        )



          };                 
                 
                 
   
                
	\legend{ ,Fault-Free, Fault, 1$\times$ Vcycle, 2$\times$ Vcycle, 3$\times$ Vcycle}
  \end{semilogyaxis}
\end{tikzpicture}


==> faultafter5iterDiffTypes.tex <==
	\pgfplotsset{tick label style ={font=\scriptsize}}
	\begin{tikzpicture}[scale=0.79]
\definecolor{darkgreen}{rgb}{0.125,0.5,0.169}
		\begin{semilogyaxis}[
		width=0.6\textwidth,
		height=0.5\textwidth,
		xlabel={Iterations},
		ylabel={Residual},
		%legend
		xticklabels = {0, 5, 5, 10, 15, 20},
		xtick = {0, 5, 8, 13, 18, 23},
		ymajorgrids = true,
		xmin = 0, xmax = 23,
		ymin=1e-16,ymax=1,
		ytick = {1e0, 1e-4, 1e-8, 1e-12,1e-16},
		%yticklabels = { $10^0$, $10^{-4}$, $10^{-8}$,\scriptsize $10^{-12}$,
		%\scriptsize $10^{-16}$},
		%yticklabels = {1e0,1e-4,1e-8,1e-12,1e-16},
		legend style={/tikz/every odd column/.style={yshift=2pt}, font=\tiny, text height = 0.4ex, legend cell align = left}
		]
\def \sh {3}
		% Before Fault
		 \addplot[color=blue, mark=o] coordinates {
		(0.0, 1                    )
		(1.0, 0.026542107          )
		(2.0, 0.0013048188         )
		(3.0, 8.07622401223097E-005)
                (4.0, 0.000006283          )
                (5.0,6.23661729007494E-007 )
                };

                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%  After Fault
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\fill[text=FAULT, blue,fill opacity=0.25, ] (axis cs:5,1e-16) rectangle (axis cs: 5+\sh,1);  
	\node[rotate=90] at (axis cs:6.5,1e-8) {\bf FAULT \& RECOVERY};             %\& RECOVERY
	%\node[coordinate, pin = {[rotate=90] right: FAULT}]  at (axis cs:6,1e-8) {};
                % No Fault
                \addplot+[color=blue,mark=o , mark options = {fill=blue}] coordinates {
                (5 +\sh, 6.23621067526521E-007)
                (6 +\sh, 7.44060374166948E-008)
                (7 +\sh, 1.00529005867452E-008)
                (8 +\sh, 1.48514026177861E-009)
                (9+\sh, 2.34532575945481E-010)
                (10+\sh, 3.89048236714878E-011)
                (11+\sh, 6.6871464992498E-012 )
                (12+\sh, 1.17919108049753E-012)
                (13+\sh, 2.11872339214339E-013)
                (14+\sh, 3.87087946717195E-014)
                (15+\sh, 7.69193235556025E-015)
                (16+\sh, 3.22732207552463E-015)
                (17+\sh, 2.963831612675E-015  )
                (18+\sh, 2.95927752680608E-015)
                (19+\sh, 2.95576030870196E-015)
                (20+\sh, 2.961322799299E-015  )
                (21+\sh, 2.961322799299E-015  )
                 };
                 
        % Fault       
        \addplot+[color=red, mark=square, mark options={solid}] coordinates { 
	      (5 +\sh, 0.1550719098		)
	      (6 +\sh, 0.0012707323             )
	      (7 +\sh, 5.97060988155311E-005    )
	      (8 +\sh, 0.000004814              )
	      (9 +\sh, 5.23915050033952E-007    )
	      (10+\sh, 6.7742433914928E-008     )
	      (11+\sh, 9.74131165805321E-009    )
	      (12+\sh, 1.50426742242806E-009    )
	      (13+\sh, 2.44211228261356E-010    )
	      (14+\sh, 4.1101438196582E-011     )
	      (15+\sh, 7.10315411107903E-012    )
	      (16+\sh, 1.25225976180504E-012    )
	      (17+\sh, 2.24183415808371E-013    )
	      (18+\sh, 4.07151541273436E-014    )
	      (19+\sh, 7.99140416292242E-015    )
	      (20+\sh, 3.25479703821773E-015    )
	      (21+\sh, 2.96864186587404E-015    )
               };
               
          %2x Vcycle
         \addplot+[color=orange,mark=triangle,mark options={solid}] coordinates { 
               (5 +\sh,      0.0001266284)
               (6 +\sh,      3.30987708034302E-006)
               (7 +\sh,      2.23706456636564E-007)
               (8 +\sh,      2.164325243054E-008)
               (9 +\sh,      2.6400442396913E-009)
               (10+\sh,      3.69697844534894E-010)
               (11+\sh,      5.62933807175125E-011)
               (12+\sh,      9.05600305774337E-012)
               (13+\sh,      1.51428234519158E-012)
               (14+\sh,      2.60529900420033E-013)
               (15+\sh,      4.58889209662794E-014)
               (16+\sh,      8.69911723924809E-015)
               (17+\sh,      3.30569708009905E-015)
               (18+\sh,      2.97055295547974E-015)
               (19+\sh,      2.95641089239752E-015)
               (20+\sh,      2.96009482257363E-015)
               (21+\sh,      2.95942797428568E-015)
                }; 
                
        % 2x Wcycle       
        \addplot+[color=green,mark=diamond,mark options={solid}] coordinates {    
              (5 +\sh,      7.49545607950133E-005)
              (6 +\sh,      2.54176137403276E-006)
              (7 +\sh,      0.000000187          )
              (8 +\sh,      0.000000018          )
              (9 +\sh,      2.06283418654674E-009)
              (10+\sh,      2.67646066205023E-010)
              (11+\sh,      3.80442234267056E-011)
              (12+\sh,      5.77909430617282E-012)
              (13+\sh,      9.20600326105077E-013)
              (14+\sh,      1.51812078899538E-013)
              (15+\sh,      2.58470396408778E-014)
              (16+\sh,      5.32238455189015E-015)
              (17+\sh,      3.05455144287265E-015)
              (18+\sh,      2.9588017874787E-015 )
              (19+\sh,      2.95962314939435E-015)
              (20+\sh,      2.95569525033241E-015)
              (21+\sh,      2.95921246843653E-015)
               }; 
         
           % 2x Fcycle
           \addplot+[solid,color=magenta, mark=pentagon,mark options={solid}] coordinates { 
               (5 +\sh,     7.50037611869899E-005)
               (6 +\sh,     0.000002541          )
               (7 +\sh,     1.869334330895E-007  )
               (8 +\sh,     0.000000018          )
               (9 +\sh,     2.06222426433216E-009)
               (10+\sh,     2.67548885265499E-010)
               (11+\sh,     3.80229574721571E-011)
               (12+\sh,     5.77413360549418E-012)
               (13+\sh,     9.19486201526432E-013)
               (14+\sh,     1.51566890169274E-013)
               (15+\sh,     2.57952775755999E-014)
               (16+\sh,     5.31429291717663E-015)
               (17+\sh,     3.05401471132382E-015)
               (18+\sh,     2.96357137919677E-015)
               (19+\sh,     2.96075353856538E-015)
               (20+\sh,     2.95863507540672E-015)
               (21+\sh,     2.95994437509403E-015)
                }; 
                                            \addplot+[solid,color=darkgreen, mark={x},mark options={solid}] coordinates {        
(5 +\sh,0.0101211306                  )
(6 +\sh,0.000208974                   )
(7 +\sh,1.34319103170376E-005         )
(8 +\sh,0.000001421                   )
(9 +\sh,1.92200314719863E-007         )
(10+\sh,2.92497956760581E-008         )
(11+\sh,4.74491019911927E-009         )
(12+\sh,8.00718081753974E-010         )
(13+\sh,1.38817482810359E-010         )
(14+\sh,2.45450996816206E-011         )
(15+\sh,4.40567146336604E-012         )
(16+\sh,8.00161019464651E-013         )
(17+\sh,1.46727767318741E-013         )
(18+\sh,2.72601074276327E-014         )
(19+\sh,5.83585773361037E-015         )
(20+\sh,3.10077541444214E-015         )
(21+\sh,2.9635266515677E-015          )

                        };
                
           % 1000x Smoothing
           \addplot+[solid,color=black, mark=asterisk,mark options={solid}] coordinates { 
           % 1500x Smoothing
%                (5 +\sh,     0.0002481893)
%                (6 +\sh,     7.16945072461411E-006)
%                (7 +\sh,     6.58605910769181E-007)
%                (8 +\sh,     9.01811128641369E-008)
%                (9 +\sh,     1.45732421398481E-008)
%                (10+\sh,     2.52457669849222E-009)
%                (11+\sh,     4.52700834404125E-010)
%                (12+\sh,     8.28056635383289E-011)
%                (13+\sh,     1.53392918137311E-011)
%                (14+\sh,     2.86639368260113E-012)
%                (15+\sh,     5.39056781769978E-013)
%                (16+\sh,     1.01901807062344E-013)
%                (17+\sh,     1.95009840438509E-014)
%                (18+\sh,     4.4977716692962E-015)
%                (19+\sh,     2.67163432605195E-015)
%                (20+\sh,     2.58027683349327E-015)
%                (21+\sh,     2.58027683349327E-015)
% 2500x Smoothing
(5 +\sh,1.46752248662188E-005)
(6 +\sh,4.45096859192271E-007)
(7 +\sh,4.26843252386916E-008)
(8 +\sh,5.91967437094387E-009)
(9 +\sh,0.000000001)
(10+\sh,1.6480579365983E-010)
(11+\sh,2.94583285893203E-011)
(12+\sh,5.37816561214034E-012)
(13+\sh,9.95563670076934E-013)
(14+\sh,1.86090824807664E-013)
(15+\sh,3.51236154259039E-014)
(16+\sh,7.11736146126445E-015)
(17+\sh,2.87152941559181E-015)
(18+\sh,2.5876815601568E-015)
(19+\sh,2.57545013906735E-015)                   
(20+\sh,2.57545013906735E-015)
(21+\sh,2.57545013906735E-015)
%                (5 +\sh,     0.0002481893)
%                (6 +\sh,     7.16945072461411E-006)
%                (7 +\sh,     6.58605910769181E-007)
%                (8 +\sh,     9.01811128641369E-008)
%                (9 +\sh,     1.45732421398481E-008)
%                (10+\sh,     2.52457669849222E-009)
%                (11+\sh,     4.52700834404125E-010)
%                (12+\sh,     8.28056635383289E-011)
%                (13+\sh,     1.53392918137311E-011)
%                (14+\sh,     2.86639368260113E-012)
%                (15+\sh,     5.39056781769978E-013)
%                (16+\sh,     1.01901807062344E-013)
%                (17+\sh,     1.95009840438509E-014)
%                (18+\sh,     4.4977716692962E-015)
%                (19+\sh,     2.67163432605195E-015)
%                (20+\sh,     2.58027683349327E-015)
%                (21+\sh,     2.58027683349327E-015)
                }; 
         

          
           \addplot+[solid,color=gray, mark={+},mark options={solid}] coordinates { 
            % 150x PCG
%                (5 +\sh,     7.80871326100747E-006)
%                (6 +\sh,     3.78328670646216E-007)
%                (7 +\sh,     4.52603243278411E-008   )
%                (8 +\sh,     6.13892910004717E-009   )
%                (9 +\sh,     9.05649712919438E-010   )
%                (10+\sh,     1.42553390478359E-010   )
%                (11+\sh,     2.35678095671834E-011   )
%                (12+\sh,     4.04069956571949E-012   )
%                (13+\sh,     7.11638555000732E-013   )
%                (14+\sh,     1.278939835071E-013   )
%                (15+\sh,     2.34753013126006E-014   )
%                (16+\sh,     5.0244791073665E-015   )
%                (17+\sh,     2.70085066931247E-015   )
%                (18+\sh,     2.58255395975993E-015   )
%                (19+\sh,     2.5770359948602E-015   )
%                (20+\sh,     2.57270538865666E-015   )
%                (21+\sh,      2.57270538865666E-015  )
% 100x PCG
 (5 +\sh, 0.0001742103		)
 (6 +\sh,  0.000006756          )
 (7 +\sh,  8.20851157268099E-007)
 (8 +\sh,  0.000000118          )
 (9 +\sh,  1.84840031879768E-008)
 (10+\sh,  3.06735820822693E-009)
 (11+\sh,  5.29765293342659E-010)
 (12+\sh,  9.41168816382297E-011)
 (13+\sh,  1.70626291049267E-011)
 (14+\sh,  3.13941705567574E-012)
 (15+\sh,  5.84038158130154E-013)
 (16+\sh,  1.09594834176412E-013)
 (17+\sh,  2.08500593679348E-014)
 (18+\sh,  4.70137115531628E-015)
 (19+\sh,  2.68470340430377E-015)
 (20+\sh,  2.57967095525447E-015)
 (21+\sh,   2.57967095525447E-015                    )
                };                          
                
                

                           
                
	\legend{,Fault-Free, Fault, 2$\times$ Vcycle, 2$\times$ Wcycle, 2$\times$ Fcycle, 15$\times$ Smth, 2000$\times$ Smth,100$\times$ PCG,}
	\end{semilogyaxis}
	\end{tikzpicture}


==> faultafter5iterDiffVcycles.tex <==
\centering
	\pgfplotsset{tick label style ={font=\scriptsize}}
	\begin{tikzpicture}[scale=0.79]
		\begin{semilogyaxis}[
		width=0.6\textwidth,
		height=0.5\textwidth,
		xlabel={Iterations},
		ylabel={Residual},
%		legend pos=south,
		xticklabels = {0, 5, 5, 10, 15, 20},
		xtick = {0, 5, 8, 13, 18, 23},
		ymajorgrids = true,
		xmin = 0, xmax = 23,
		ymin=1e-16,ymax=1,
		ytick = {1e0, 1e-4, 1e-8, 1e-12, 1e-16},
		%yticklabels = {\scriptsize $10^0$,\scriptsize $10^{-4}$,\scriptsize $10^{-8}$,\scriptsize $10^{-12}$,
		%\scriptsize $10^{-16}$},
		legend style={/tikz/every odd column/.style={yshift=2pt}, font=\scriptsize, text height = 0.5ex, legend cell align = left},
%		every axis label/.append style = {font=\tiny}
		]
\def \sh {3}
		% Before Fault
		 \addplot[color=blue,mark=o] coordinates {
		(0.0, 1                    )
		(1.0, 0.026542107          )
		(2.0, 0.0013048188         )
		(3.0, 8.07622401223097E-005)
                (4.0, 0.000006283          )
                (5.0,6.23661729007494E-007 )
                };

                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%  After Fault
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\fill[text=FAULT, blue,fill opacity=0.25, ] (axis cs:5,1e-16) rectangle (axis cs: 5+\sh,1);  
	\node[rotate=90] at (axis cs:6.5,1e-8) { \bf FAULT \& RECOVERY};             %
	%\node[coordinate, pin = {[rotate=90] right: FAULT}]  at (axis cs:6,1e-8) {};
                % No Fault
                \addplot+[color=blue,mark=o , mark options = {fill=blue}] coordinates {
                (5 +\sh, 6.23621067526521E-007)
                (6 +\sh, 7.44060374166948E-008)
                (7 +\sh, 1.00529005867452E-008)
                (8 +\sh, 1.48514026177861E-009)
                (9+\sh, 2.34532575945481E-010)
                (10+\sh, 3.89048236714878E-011)
                (11+\sh, 6.6871464992498E-012 )
                (12+\sh, 1.17919108049753E-012)
                (13+\sh, 2.11872339214339E-013)
                (14+\sh, 3.87087946717195E-014)
                (15+\sh, 7.69193235556025E-015)
                (16+\sh, 3.22732207552463E-015)
                (17+\sh, 2.963831612675E-015  )
                (18+\sh, 2.95927752680608E-015)
                (19+\sh, 2.95576030870196E-015)
                (20+\sh, 2.961322799299E-015  )
                (21+\sh, 2.961322799299E-015  )
                 };
                 
        % Fault       
        \addplot+[color=red, mark=square, mark options={solid}] coordinates { 
	      (5 +\sh, 0.1550719098		)
	      (6 +\sh, 0.0012707323             )
	      (7 +\sh, 5.97060988155311E-005    )
	      (8 +\sh, 0.000004814              )
	      (9 +\sh, 5.23915050033952E-007    )
	      (10+\sh, 6.7742433914928E-008     )
	      (11+\sh, 9.74131165805321E-009    )
	      (12+\sh, 1.50426742242806E-009    )
	      (13+\sh, 2.44211228261356E-010    )
	      (14+\sh, 4.1101438196582E-011     )
	      (15+\sh, 7.10315411107903E-012    )
	      (16+\sh, 1.25225976180504E-012    )
	      (17+\sh, 2.24183415808371E-013    )
	      (18+\sh, 4.07151541273436E-014    )
	      (19+\sh, 7.99140416292242E-015    )
	      (20+\sh, 3.25479703821773E-015    )
	      (21+\sh, 2.96864186587404E-015    )
               };
        % 1x Vcycle       
        \addplot+[color=green,mark=triangle,mark options={solid}] coordinates {    
              (5 +\sh,      0.003175373)
              (6 +\sh,      0.000057451)
              (7 +\sh,      3.38273025580138E-006)
              (8 +\sh,      2.9567361842453E-007)
              (9 +\sh,      3.3397348058211E-008)
              (10+\sh,      4.41949636689668E-009)
              (11+\sh,      6.46407761463488E-010)
              (12+\sh,      1.0101857009836E-010)
              (13+\sh,      1.65292173071528E-011)
              (14+\sh,      2.79613959899647E-012)
              (15+\sh,      4.84957285114238E-013)
              (16+\sh,      8.57843396372183E-014)
              (17+\sh,      1.56634937157681E-014)
              (18+\sh,      4.06337498424368E-015)
              (19+\sh,      3.00041068095782E-015)
              (20+\sh,      2.96145291603811E-015)
              (21+\sh,      2.95942797428568E-015)
               }; 
               
          %2x Vcycle
         \addplot+[color=orange,mark=diamond,mark options={solid}] coordinates { 
               (5 +\sh,      0.0001266284)
               (6 +\sh,      3.30987708034302E-006)
               (7 +\sh,      2.23706456636564E-007)
               (8 +\sh,      2.164325243054E-008)
               (9 +\sh,      2.6400442396913E-009)
               (10+\sh,      3.69697844534894E-010)
               (11+\sh,      5.62933807175125E-011)
               (12+\sh,      9.05600305774337E-012)
               (13+\sh,      1.51428234519158E-012)
               (14+\sh,      2.60529900420033E-013)
               (15+\sh,      4.58889209662794E-014)
               (16+\sh,      8.69911723924809E-015)
               (17+\sh,      3.30569708009905E-015)
               (18+\sh,      2.97055295547974E-015)
               (19+\sh,      2.95641089239752E-015)
               (20+\sh,      2.96009482257363E-015)
               (21+\sh,      2.95942797428568E-015)
                }; 
         
           % 3x Vcycle
           \addplot+[solid,color=magenta, mark=pentagon,mark options={solid}] coordinates { 
               (5 +\sh,     6.59931770034928E-006)
               (6 +\sh,     2.26571057971073E-007)
               (7 +\sh,     1.97781509598143E-008)
               (8 +\sh,     2.39451801913529E-009)
               (9 +\sh,     3.41564572464858E-010)
               (10+\sh,     5.31953824822208E-011)
               (11+\sh,     8.74925284528713E-012)
               (12+\sh,     1.49339047626793E-012)
               (13+\sh,     2.61762349908308E-013)
               (14+\sh,     4.68753684946713E-014)
               (15+\sh,     8.982731069031E-015)
               (16+\sh,     3.3332330350136E-015)
               (17+\sh,     2.96843042617298E-015)
               (18+\sh,     2.95890750732923E-015)
               (19+\sh,     2.96090805219308E-015)
               (20+\sh,     2.96068848019583E-015)
               (21+\sh,     2.96114388878272E-015)
                }; 
         
	\legend{ ,Fault-Free, Fault, 1$\times$ Vcycle, 2$\times$ Vcycle, 3$\times$ Vcycle}
	\end{semilogyaxis}
	\end{tikzpicture}

